Tractable Compositions of Discrete-Time Control Barrier Functions with Application to Lane Keeping and Obstacle Avoidance

This paper introduces control barrier functions for discrete-time systems, which can be shown to be necessary and sufficient for controlled invariance of a given set. Moreover, we propose nonlinear discrete-time control barrier functions for partially control affine systems that lead to controlled invariance conditions that are affine in the control input, leading to a tractable formulation that enables us to handle the safety optimal control problem for a broader range of applications with more complicated safety conditions than existing approaches. In addition, we develop mixed-integer formulations for basic and secondary Boolean compositions of multiple control barrier functions and further provide mixed-integer constraints for piecewise control barrier functions. Finally, we apply these discrete-time control barrier function tools to automotive safety problems of lane keeping and obstacle avoidance, which are shown to be effective in simulation.

==> sec_model2.tex <==
%!TEX root = main.tex
\subsection{Modeling Framework} \label{sec:model}
\begin{remark}
\end{remark}

\begin{remark}
\end{remark}

\begin{example}

\end{example}


==> sec_motivation.tex <==
%!TEX root = main.tex
%\section{Motivating Example: Intention-Aware Vehicles} \label{sec:motivation}

%\begin{figure}[!h]
%\begin{center}
%\includegraphics[width=2in]{Figures/Intersection4way2.png}
%\caption{Two vehicles crossing a 4-way intersection.\label{fig:intersection} }
%\end{center}
%\end{figure}

%To motivate the input design problem studied in this paper, we consider the scenario of vehicles crossing an intersection, where each vehicle does not have any information about the intention of the other vehicles.
%To simplify the problem, we consider the case with two vehicles (see Fig. \ref{fig:intersection}). 
%The controlled/ego vehicle (in blue) can choose any control input subject to engine power and braking limitations, as long as traffic laws are obeyed. 
%Vehicle A is human driven (uncontrolled) and Vehicle B is autonomous (controlled), with dynamics described by $\ddot{x}_A=-0.1\dot{x}_A + d_1$ and $\ddot{x}_B=-0.1\dot{x}_B + u$, where $x$ and $\dot{x}$ are vehicle positions and velocities.
%At the intersection, 
%On the other hand, the driver of the other vehicle (in red)---autonomous or human-driven---can choose between three intentions\footnote{The assumed intentions (also used in \cite{Yong2014}) are for illustrative purposes only; the proposed approach is also applicable with other intention models.}:
%\begin{itemize}
%\item to fail to notice the ego vehicle, thus proceeding with any unknown control input that maintains the velocity within a desired range to ensure forward mobility (Inattentive Driver),
%\item to attempt to cause a collision (Malicious Driver), or
%\item to stop (Cautious Driver).
%\end{itemize}
%In this case, we have two \emph{rational} agents, each with \emph{individual responsibilities}. Both vehicles have to individually satisfy velocity restrictions imposed by traffic laws and by the assumption of forward mobility, respectively. This model of individual responsibilities is an appropriate model of interactions between rational agents, since the ego vehicle should not be responsible for choosing an input that ensures the constraint satisfaction of the other vehicle and vice versa.

%The objective is to 
%%actively 
%identify the intention of other \emph{rational} drivers at intersections by taking appropriate control actions while %simultaneously 
%optimizing for safety, comfort or energy efficiency.
